Interpretable Data-Based Explanations for Fairness Debugging

A wide variety of fairness metrics and eXplainable Artificial Intelligence (XAI) approaches have been proposed in the literature to identify bias in machine learning models that are used in critical real-life contexts. However, merely reporting on a model's bias, or generating explanations using existing XAI techniques is insufficient to locate and eventually mitigate sources of bias. We introduce Gopher, a system that produces compact, interpretable and causal explanations for bias or unexpected model behavior by identifying coherent subsets of the training data that are root-causes for this behavior. Specifically, we introduce the concept of causal responsibility that quantifies the extent to which intervening on training data by removing or updating subsets of it can resolve the bias. Building on this concept, we develop an efficient approach for generating the top-k patterns that explain model bias that utilizes techniques from the machine learning (ML) community to approximate causal responsibility and uses pruning rules to manage the large search space for patterns. Our experimental evaluation demonstrates the effectiveness of Gopher in generating interpretable explanations for identifying and debugging sources of bias.

==> feedback.tex <==
1. Once we define individual level causes, we define predicate level causation (the idea of summarization). (this might be a difference from PrIU)

2. Then we extend the definition over an aggregate over a set of individual decisions.

3. Finally, we connect causation to provenance

By arguing the annotation for data points in the training data serve as provenance for ML decisions

for provenance definitions: 
1. "The Complexity of Causality and Responsibility for Query Answers and non-Answers"

2. Sudeepa, Suciu -- explaining aggregates

When aggregates, measure the effect of a tuple or tuples on the value of the aggregated quantity

==> influence-lr.tex <==
\section{Influence Computation for Logistic Regression}


